Data and Representation for Turkish Natural Language Inference

Large annotated datasets in NLP are overwhelmingly in English. This is an obstacle to progress in other languages. Unfortunately, obtaining new annotated resources for each task in each language would be prohibitively expensive. At the same time, commercial machine translation systems are now robust. Can we leverage these systems to translate English-language datasets automatically? In this paper, we offer a positive response for natural language inference (NLI) in Turkish. We translated two large English NLI datasets into Turkish and had a team of experts validate their translation quality and fidelity to the original labels. Using these datasets, we address core issues of representation for Turkish NLI. We find that in-language embeddings are essential and that morphological parsing can be avoided where the training set is large. Finally, we show that models trained on our machine-translated datasets are successful on human-translated evaluation sets. We share all code, models, and data publicly.

==> tables/cs1_app.tex <==
\begin{table*}[!ht]\centering
\setlength{\tabcolsep}{12pt}
\begin{tabular}{lllll}
\toprule
\textbf{}  &\textbf{SNLI} &\multicolumn{2}{c}{\textbf{MultiNLI}} \\\cmidrule{2-4}
\textbf{Model Name} & \textbf{Test} & \textbf{Matched Dev} &\textbf{Mismatched Dev} \\\midrule
\textbf{\BertEn\ (Cased)} & \textbf{90.13\%} & \textbf{83.16\%} &  \textbf{83.95\%} \\
\textbf{\BertEn\ (Uncased)} &89.70\% & 80.23\% & 81.17\% \\ \midrule

\textbf{\BertMultilingual\ (Cased)} &89.02\% & 81.74\% & 82.13\% \\
\textbf{\BertMultilingual\ (Uncased)} &87.98\% & 78.45\% & 78.99\% \\ \midrule

\textbf{BERTurk (Cased)} &85.84\% & 75.16\% & 75.60\% \\
\textbf{BERTurk (Uncased)} &85.06\% & 32.74\% & 35.22\% \\
\bottomrule
\end{tabular}
\caption{Accuracy of the models in \Tabref{tab:case_study_i_results_table} trained on SNLI and MultiNLI. We used the same fine-tuning and evaluation procedures. \BertEn\ ranked the first and \BertMultilingual\ ranked the second, emphasizing the importance of in-language training one-more time. Similarly, casing enhanced the models as in \Secref{sec:case-study-i}. Overall, the outcomes agree with the previous ones.}.
\label{tab:case_study_i_app_table}
\end{table*}

